Graph Adversarial Diffusion Convolution

This paper introduces a min-max optimization formulation for the Graph Signal Denoising (GSD) problem. In this formulation, we first maximize the second term of GSD by introducing perturbations to the graph structure based on Laplacian distance and then minimize the overall loss of the GSD. By solving the min-max optimization problem, we derive a new variant of the Graph Diffusion Convolution (GDC) architecture, called Graph Adversarial Diffusion Convolution (GADC). GADC differs from GDC by incorporating an additional term that enhances robustness against adversarial attacks on the graph structure and noise in node features. Moreover, GADC improves the performance of GDC on heterophilic graphs. Extensive experiments demonstrate the effectiveness of GADC across various datasets. Code is available at https://github.com/SongtaoLiu0823/GADC.

==> 05related_work.tex <==
Several defense methods~\citep{wu2019adversarial,zugner2019robustgcn,entezari2020all} have recently been proposed to counter graph structure attacks. By utilizing the insertion term in our proposed GADC, we can reconstruct the informative adjacency matrix, thus restoring efficient information flow and defending against adversarial structure attacks. Existing graph denoising works primarily focus on graph smoothing techniques~\citep{chen2014signal,zhou2021graph}. Some recent GNN models, such as S$^2$GC~\citep{zhu2021simple}, GLP~\citep{li2019label}, and IRLS~\citep{yang2021graph}, are derived from the perspective of signal denoising. Additionally, \citet{ma2021unified} connect signal denoising to popular GNNs. Further discussion about related work can be found in Appendix~\ref{appendix:related}.
